ClavaDDPM: Multi-relational Data Synthesis with Cluster-guided Diffusion Models

Recent research in tabular data synthesis has focused on single tables, whereas real-world applications often involve complex data with tens or hundreds of interconnected tables. Previous approaches to synthesizing multi-relational (multi-table) data fall short in two key aspects: scalability for larger datasets and capturing long-range dependencies, such as correlations between attributes spread across different tables. Inspired by the success of diffusion models in tabular data modeling, we introduce $\textbf{C}luster$ $\textbf{La}tent$ $\textbf{Va}riable$ $guided$ $\textbf{D}enoising$ $\textbf{D}iffusion$ $\textbf{P}robabilistic$ $\textbf{M}odels$ (ClavaDDPM). This novel approach leverages clustering labels as intermediaries to model relationships between tables, specifically focusing on foreign key constraints. ClavaDDPM leverages the robust generation capabilities of diffusion models while incorporating efficient algorithms to propagate the learned latent variables across tables. This enables ClavaDDPM to capture long-range dependencies effectively. Extensive evaluations on multi-table datasets of varying sizes show that ClavaDDPM significantly outperforms existing methods for these long-range dependencies while remaining competitive on utility metrics for single-table data.

==> outline.tex <==
Background:
- The standard definition of multi-relational databases:
R1,R2,... attributes, domain
Person = {p1, p2, ...}
Household = {h1, h2, ...}

foreign-key relationship constraint 
running example 
*DAG based on FK constraints 
* (optional) other general constraints 

- Multi-relational synthesis 
given a multi-relational database, what properties are required to be learned/preserved in its synthetic version? most single-table syntheses only captures the inter-table correlations, but not the others.
*a summary of the important properties of PrivLava 
*metrics used in the evaluation? (optional)  

- Problem statement: 

Sec 4 ClavaDDPM:

- Model multi-relational DB
  * model 2-table cases: 
        - Household-person attributes: level-1 attribute, level-2 attribute; [notations]
        - full joint distribution for household-person, and how it catpures the properties defined in the background
        - independent assumptions; modeling the level-2 attributes with cardianlity and other parameters to simplify the expression with additional assumptions; ]
        - differences from PrivLava [altnerative: at related work]: (i) theoretical framework with explicit independent assumption stated; (ii) how we capture the latent variable (we do explicitly clustering, why is this good?) (iii) our model is more general than theirs (give a head up) we will elaborate more in later section
        
  * how to generalize to more complex cases 

- Generative process 

  
  
g = {x1, ..., xn}

G = f(X, S)

G_s = f(X, s)

g g_s


==> todos.tex <==
*improve the contribution in intro
*shorten sec 4
*shorten sec 5

